Dataset Distillation

Model distillation aims to distill the knowledge of a complex model into a simpler one. In this paper, we consider an alternative formulation called dataset distillation: we keep the model fixed and instead attempt to distill the knowledge from a large training dataset into a small one. The idea is to synthesize a small number of data points that do not need to come from the correct data distribution, but will, when given to the learning algorithm as training data, approximate the model trained on the original data. For example, we show that it is possible to compress 60,000 MNIST training images into just 10 synthetic distilled images (one per class) and achieve close to original performance with only a few gradient descent steps, given a fixed network initialization. We evaluate our method in various initialization settings and with different learning objectives. Experiments on multiple datasets show the advantage of our approach compared to alternative methods.

==> figText/adapt.tex <==
%auto-ignore
%!TEX root = ../main.tex

\begin{figure}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.85\textwidth]{figures/adapt}
    \caption{We train $100$ \images applied in $10$ steps and $3$ epochs for each fast domain adaptation task. Images in last steps are visualized. From top to bottom: \mnist $\rightarrow$ \usps, \usps $\rightarrow$ \mnist, \svhn $\rightarrow$ \mnist. }
    \lblfig{adapt}
    \vspace{-5pt}
\end{figure}


==> figText/forget.tex <==
%auto-ignore
%!TEX root = ../main.tex

\begin{figure}
    \centering
    % \vspace{-5pt}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/forget_mnist.pdf}
        \caption{\mnist. Attacked category: $0$. Target category: $1$.}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/forget_cifar.pdf}
        \caption{\cifar{10}. Attacked category: {\tt plane}. Target category: {\tt car}.}
    \end{subfigure}
    \caption{Malicious \images can manipulate well-trained neural network models to misclassify attacked category images as the target category with one GD step and $10$ images. These images are trained with $2000$ well-optimized neural network models and evaluated on $200$ held-out models. Better results with larger batch size can be found at \reftbl{forget}. }
    \lblfig{forget}
    \vspace{-10pt}
\end{figure}


==> figText/init.tex <==
%auto-ignore
%!TEX root = ../main.tex

\begin{figure}
    \centering
    \vspace{-1pt}\hfill%
    \includegraphics[scale=0.35]{figures/init/MNIST_LeNet5_ExtendedSimpleResNet2.png}\hfill%
    \includegraphics[scale=0.35]{figures/init/Cifar10_VGG11_VGG19.png}\hfill
    \includegraphics[scale=0.35]{figures/init/Cifar10_VGG11_ResNet18.png}\hfill
    \vspace{-10pt}
    \caption{Compare our network initialization method on \mnist and \cifar{10} against ``\xavier'', ``\kaiming'' and a data-dependent initialization (``DDI'' in plot). While the \images are trained on small networks (\ie, \lenet and \vgg{11}), they can speed up training on much larger networks. The experiment is done with SGD using batch size $256$ and learning rate $0.01$. For a fair comparison, the plots are made so that each iteration processes the same amount of data, regardless of real or synthetic. }
    \lblfig{init}
\end{figure}


==> figText/table-charge-one-vs-N-steps.tex <==
%auto-ignore
%!TEX root = ../main.tex

\begin{table}[th]
\vspace{-5pt}
\centering
\resizebox{0.75\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c||c|c||c||c|}
    \hline
    & \multirow{2}{*}{\shortstack{$N$\\(\#images per category)}}
    & \multirow{2}{*}{\shortstack{Total \#images\\($N \times \text{\#categories}$)}}
    & \multirow{2}{*}{Applied in 1 GD step}
    & \multirow{2}{*}{Applied in $N$ GD steps} \\
    & & & & \\
    \hline

    \multirow{5}{*}{\mnist}
    & $1$ & $10$
    & $\musigpb{19.81}{5.83}$ & $\musigpb{19.81}{5.83}$ \\
    \cline{2-5}
    & $5$ & $50$
    & $\musigp{21.19}{5.47}$ & $\musigpb{53.94}{9.45}$  \\
    \cline{2-5}
    & $10$ & $100$
    & $\musigp{21.45}{5.81}$ & $\musigpb{69.32}{8.86}$ \\
    \cline{2-5}
    & $20$ & $200$
    & $\musigp{21.49}{5.96}$ & $\musigpb{72.68}{12.44}$ \\
    \cline{2-5}
    & $30$ & $300$
    & $\musigp{21.57}{5.91}$ & $\musigpb{83.58}{5.08}$ \\
    \hline
    \multirow{5}{*}{\cifar{10}}
    & $1$ & $10$
    & $\musigpb{17.95}{2.41}$ & $\musigpb{17.95}{2.41}$ \\
    \cline{2-5}
    & $5$ & $50$
    & $\musigp{18.25}{2.51}$ & $\musigpb{32.49}{1.28}$ \\
    \cline{2-5}
    & $10$ & $100$
    & $\musigp{18.46}{2.58}$ & $\musigpb{34.54}{1.55}$ \\
    \cline{2-5}
    & $20$ & $200$
    & $\musigp{18.58}{2.58}$ & $\musigpb{37.84}{1.63}$  \\
    \cline{2-5}
    & $30$ & $300$
    & $\musigp{18.59}{2.56}$ & $\musigpb{38.20}{1.47}$  \\
    \hline
\end{tabular}
}\vspace{-7pt}%
\caption{Comparison between applying the same number of images in one GD step versus multiple steps, with the number of epochs fixed to $1$. $N$ denotes the total number of images per category. For multiple steps runs, each of the $N$ steps applies one image per category. Using multiple steps drastically improves the performance. }
\lbltbl{charge-1-vs-n}
\vspace{-5pt}
\end{table}


==> figText/table-forget.tex <==
%auto-ignore
%!TEX root = ../main.tex

\begin{table}[th]
\centering
\resizebox{1.0\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.25}

\begin{tabular}{|c||c||c|c||c|c||c|c|}
    \hline
    & \multirow{3}{*}{\#images} &
    \multicolumn{2}{c||}{Ours} &
    \multicolumn{2}{c||}{Random real} &
    \multicolumn{2}{c|}{Optmized real} \\
    \cline{3-8}

     & &
     \multirow{2}{*}{\shortstack{Attacked cls\\predicted as target cls}} & \multirow{2}{*}{\shortstack{Overall accuracy\\\wrt \textbf{incorrect} labels}} &
     \multirow{2}{*}{\shortstack{Attacked cls\\predicted as target cls}} & \multirow{2}{*}{\shortstack{Overall accuracy\\\wrt \textbf{incorrect} labels}} &
     \multirow{2}{*}{\shortstack{Attacked cls\\predicted as target cls}} & \multirow{2}{*}{\shortstack{Overall accuracy\\\wrt \textbf{incorrect} labels}} \\
    & & & & & & & \\
    \hline

    \multirow{5}{*}{\shortstack{\mnist:\\$0 \rightarrow 1$}}
    & $10$
    & $\musigpb{65.13}{30.44}$ & $\musigpb{91.88}{4.25}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.84}{0.52}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.84}{0.52}$ \\
    \cline{2-8}
    & $50$
    & $\musigpb{70.32}{31.16}$ & $\musigpb{90.71}{5.59}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.87}{0.50}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.87}{0.50}$ \\
    \cline{2-8}
    & $100$
    & $\musigpb{71.45}{29.68}$ & $\musigpb{90.87}{5.28}$
    & $\musigp{0.02}{0.04}$ & $\musigp{88.88}{0.50}$
    & $\musigp{0.02}{0.04}$ & $\musigp{88.88}{0.50}$ \\
    \cline{2-8}
    & $200$
    & $\musigpb{71.43}{30.74}$ & $\musigpb{89.62}{6.88}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$ \\
    \cline{2-8}
    & $300$
    & $\musigpb{72.98}{30.78}$ & $\musigpb{89.15}{7.71}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$
    & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$ \\
    \hline
    \multirow{5}{*}{\shortstack{\cifar{10}:\\\tt{plane}$\rightarrow$\tt{car}}}
    & $10$
    & $\musigpb{33.23}{14.37}$ & $\musigpb{69.59}{2.03}$
    & $\musigp{3.05}{0.86}$ & $\musigp{68.71}{1.67}$
    & $\musigp{3.05}{0.86}$ & $\musigp{68.71}{1.67}$ \\
    \cline{2-8}
    & $50$
    & $\musigpb{42.39}{17.13}$ & $\musigpb{70.36}{2.12}$
    & $\musigp{3.01}{0.60}$ & $\musigp{69.69}{1.09}$
    & $\musigp{3.01}{0.60}$ & $\musigp{69.69}{1.09}$ \\
    \cline{2-8}
    & $100$
    & $\musigpb{45.92}{18.11}$ & $\musigpb{70.39}{2.39}$
    & $\musigp{3.01}{0.56}$ & $\musigp{69.96}{1.03}$
    & $\musigp{3.01}{0.56}$ & $\musigp{69.96}{1.03}$ \\
    \cline{2-8}
    & $200$
    & $\musigpb{45.58}{19.05}$ & $\musigp{69.90}{3.20}$
    & $\musigp{3.03}{0.51}$ & $\musigpb{70.08}{1.01}$
    & $\musigp{3.03}{0.51}$ & $\musigpb{70.08}{1.01}$ \\
    \cline{2-8}
    & $300$
    & $\musigpb{47.77}{18.43}$ & $\musigp{70.09}{2.76}$
    & $\musigp{3.02}{0.49}$ & $\musigpb{70.11}{1.00}$
    & $\musigp{3.02}{0.49}$ & $\musigpb{70.11}{1.00}$ \\
    \hline
\end{tabular}
}%
\caption{Fast data poisoning attack performance for our method and baseline. \Images are trained for one GD step. For baselines, we use the same numbers of randomly sampled real images with incorrect labels and also apply one GD step, and report the result that achieves the highest accuracy \wrt the incorrect labels. Our attack images are always better at changing the prediction for images of the attacked class.}
\lbltbl{forget}
\end{table}

% NOTE: Do not delete the following. We don't have the test outputs anymore. This the only place we still have these numbers.
%
% \begin{tabular}{|c||c||c|c|c||c|c|c|}
%     \hline
%     & \multirow{3}{*}{\#images} & \multicolumn{3}{c||}{Ours} &\multicolumn{3}{c|}{ Random real images} \\
%     \cline{3-8}
%      & & \multirow{2}{*}{\shortstack{Attacked class\\classified \textbf{correctly}}} &
%          \multirow{2}{*}{\shortstack{Attacked class\\classified \textbf{as target class}}} &
%          \multirow{2}{*}{\shortstack{Overall accuracy\\\wrt \textbf{incorrect} labels}}
%      &   \multirow{2}{*}{\shortstack{Attacked class\\classified \textbf{correctly}}} &
%          \multirow{2}{*}{\shortstack{Attacked class\\classified \textbf{as target class}}} &
%          \multirow{2}{*}{\shortstack{Overall accuracy\\\wrt \textbf{incorrect} labels}}\\
%     & & & & & & & \\
%     \hline

%     \multirow{5}{*}{\shortstack{\mnist:\\$0 \rightarrow 1$}}
%     & $10$
%     & $\musigpb{4.71}{12.31}$ & $\musigpb{65.13}{30.44}$ & $\musigpb{91.88}{4.25}$
%     & $\musigp{98.74}{0.38}$ & $\musigp{0.02}{0.05}$ & $\musigp{88.84}{0.52}$ \\
%     \cline{2-8}
%     & $50$
%     & $\musigpb{2.88}{8.35}$ & $\musigpb{70.32}{31.16}$ & $\musigpb{90.71}{5.59}$
%     & $\musigp{98.80}{0.33}$ & $\musigp{0.02}{0.05}$ & $\musigp{88.87}{0.50}$ \\
%     \cline{2-8}
%     & $100$
%     & $\musigpb{2.55}{8.90}$ & $\musigpb{71.45}{29.68}$ & $\musigpb{90.87}{5.28}$
%     & $\musigp{98.81}{0.33}$ & $\musigp{0.02}{0.04}$ & $\musigp{88.88}{0.50}$ \\
%     \cline{2-8}
%     & $200$
%     & $\musigpb{1.74}{7.28}$ & $\musigpb{71.43}{30.74}$ & $\musigpb{89.62}{6.88}$
%     & $\musigp{98.80}{0.33}$ & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$ \\
%     \cline{2-8}
%     & $300$
%     & $\musigpb{1.61}{7.66}$ & $\musigpb{72.98}{30.78}$ & $\musigpb{89.15}{7.71}$
%     & $\musigp{98.80}{0.34}$ & $\musigp{0.02}{0.05}$ & $\musigp{88.88}{0.50}$ \\
%     \hline
%     \multirow{5}{*}{\shortstack{\cifar{10}:\\\tt{plane}$\rightarrow$\tt{car}}}
%     & $10$
%     & $\musigpb{26.63}{9.94}$ & $\musigpb{33.23}{14.37}$ & $\musigpb{69.59}{2.03}$
%     & $\musigp{77.81}{4.45}$ & $\musigp{3.05}{0.86}$ & $\musigp{68.71}{1.67}$ \\
%     \cline{2-8}
%     & $50$
%     & $\musigpb{12.41}{8.15}$ & $\musigpb{42.39}{17.13}$ & $\musigpb{70.36}{2.12}$
%     & $\musigp{78.93}{2.23}$ & $\musigp{3.01}{0.60}$ & $\musigp{69.69}{1.09}$ \\
%     \cline{2-8}
%     & $100$
%     & $\musigpb{9.23}{6.69}$ & $\musigpb{45.92}{18.11}$ & $\musigpb{70.39}{2.39}$
%     & $\musigp{79.31}{1.59}$ & $\musigp{3.01}{0.56}$ & $\musigp{69.96}{1.03}$ \\
%     \cline{2-8}
%     & $200$
%     & $\musigpb{7.96}{6.58}$ & $\musigpb{45.58}{19.05}$ & $\musigp{69.90}{3.20}$
%     & $\musigp{79.57}{1.47}$ & $\musigp{3.03}{0.51}$ & $\musigpb{70.08}{1.01}$ \\
%     \cline{2-8}
%     & $300$
%     & $\musigpb{7.15}{6.26}$ & $\musigpb{47.77}{18.43}$ & $\musigp{70.09}{2.76}$
%     & $\musigp {79.69}{1.43}$ & $\musigp{3.02}{0.49}$ & $\musigpb{70.11}{1.00}$ \\
%     \hline
% \end{tabular}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

